Certified Robustness to Adversarial Examples with Differential Privacy

Adversarial examples that fool machine learning models, particularly deep neural networks, have been a topic of intense research interest, with attacks and defenses being developed in a tight back-and-forth. Most past defenses are best effort and have been shown to be vulnerable to sophisticated attacks. Recently a set of certified defenses have been introduced, which provide guarantees of robustness to norm-bounded attacks, but they either do not scale to large datasets or are limited in the types of models they can support. This paper presents the first certified defense that both scales to large networks and datasets (such as Google's Inception network for ImageNet) and applies broadly to arbitrary model types. Our defense, called PixelDP, is based on a novel connection between robustness against adversarial examples and differential privacy, a cryptographically-inspired formalism, that provides a rigorous, generic, and flexible foundation for defense.

==> Makefile <==
PAPER=paper
LATEX=pdflatex

BIBTEX=bibtex

SRCS=$(PAPER).tex $(wildcard sections/*.tex)
REFS=$(wildcard bib/*.bib)
FIGS=$(wildcard figures/*)
STYLE=$(wildcard style/*)

.PHONY: results $(PAPER).pdf clean

# all: $(PAPER).pdf

arxiv:
	$(LATEX) $(PAPER)

arxiv-clean:
	rm -f *.dvi *.aux *.log *.blg \
          $(PAPER).ps $(PAPER).pdf \
          $(PAPER)-single.pdf $(PAPER)-single.ps

results:
	+make -C $@

$(PAPER).pdf: $(SRCS) $(REFS) $(FIGS) $(STYLE)
	$(LATEX) $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX) $(PAPER)


submission: $(PAPER).pdf
	cp $(PAPER).pdf submission/

# clean:
	# rm -f *.dvi *.aux *.log *.blg *.bbl \
          # $(PAPER).ps $(PAPER).pdf \
          # $(PAPER)-single.pdf $(PAPER)-single.ps

